Understanding Generative AI Content with Embedding Models

Constructing high-quality features is critical to any quantitative data analysis. While feature engineering was historically addressed by carefully hand-crafting data representations based on domain expertise, deep neural networks (DNNs) now offer a radically different approach. DNNs implicitly engineer features by transforming their input data into hidden feature vectors called embeddings. For embedding vectors produced by foundation models -- which are trained to be useful across many contexts -- we demonstrate that simple and well-studied dimensionality-reduction techniques such as Principal Component Analysis uncover inherent heterogeneity in input data concordant with human-understandable explanations. Of the many applications for this framework, we find empirical evidence that there is intrinsic separability between real samples and those generated by artificial intelligence (AI).

==> science_template/old_results_section.tex <==
Our findings suggest that the highest degrees of variability are correlated with intuitive differences in the samples, such as variation in the subject area or the source of the content. More nuanced differences can arise from semantics in natural language such as differences in the vocabulary of a prompted language model. We show that different generative models and prompting techniques can be identified from their outputs. For textual data, we use linear regression on explanatory variables to relate the observed variation to structures in the underlying texts.

\subsubsection*{High-level semantics}

The vector representations created by FEs encode more than simple combinations of attributes of the underlying data. Across datasets, Fig.~\ref{fig:MAIN1}B,C shows that the features encoded by the top principal components (PCs) of FE vector representations can have simple interpretations that agree with human intuition. For example, examining FE vectors of academic abstracts from both the arXiv and \texttt{Llama-2 70B} across five subject areas, we find that the top three principal components of the data cluster articles according to their respective fields (Fig. \ref{fig:MAIN1}B, right). In this case, the clustering is independent of the origin of the articles. 

However, looking at Spanish and Russian news articles from the MLSUM dataset (Fig. \ref{fig:MAIN1}B, left), along with machine translations of these Russian articles into Spanish, we find that the principle components are sensitive to the origin of the data, even when the content is similar. Articles in the two different languages separate along PC1 and, akin to the arXiv abstracts, the topics (sports and economics) separate along PC2. PC3, however, separates the Spanish articles by their origin: native versus machine-translated. Using clustering techniques by non-negative matrix factorization, we observe in Fig.~\ref{fig:nmf_mlsum_factors} that the separation between the native Spanish articles and those that were machine translated are likely a compounded effect of the quality of translation and other natural semantic variation between Spanish and Russian cultures and patterns (e.g. the discussion of Rubles or Euro in the text). Furthermore, with the exclusion of machine translated articles, PC3 spreads out as a linear combination of the new features (Fig.~\ref{fig:PCA_comparison}). Regressions explaining the clusters in terms these metadata attributes are in Fig. \ref{tab:regressions}.

In the next section we dig deeper into what embedding models can tell us about the origin of the data.


\subsubsection*{AI-generated data is shifted from real}\label{section:real_fake}
Across the examples presented in Fig.~\ref{fig:MAIN2}, we find that FEs numerically encode raw data in a way that enables the identification of hyperplanes in the ambient vector space that separate the subspaces corresponding to AI-generated and real content. Comparing abstracts of papers from five different subjects on the arXiv and corresponding abstracts generated using \texttt{Llama-2 70B}, we discover that the differences between the real and AI-generated abstracts explain the uniform separation observed along the direction of PC4 of the embedded text $(R^2=0.79)$. Further, supervised learning on the embedded data can find a universal separator in the ambient vector space that distinguishes the classes of real and fake data, obtaining $99.9\pm0.13\%$ test accuracy. When we consider a UMAP of the top 30 PCs (chosen using Scree plots in Fig.~\ref{fig:scree1}), we find considerable overlap between the real and fake clusters of data. This indicates that while simple decision boundaries exist to separate different kinds of data, the text produced by the LLM may still reflect human writing reasonably well according to the vectorized text. 

%Across the examples in Fig.~\ref{fig:MAIN2}, we find that embeddings of AI-generated data is shifted from those of real baselines. In the five subject arXiv abstracts, PC4 is explained by the clustering of arXiv abstracts and those generated by \texttt{Llama-2 70B} ($R^2 = 0.79$), independent of the subject area. A simple LDA classifier separates these samples even further, achieving $99.9 \pm 0.13\%$ test accuracy when classifying real/AI-generated abstracts across all five topics. Fig.~\ref{fig:MAIN2}B suggests a subtlety in this result. When considering the signal of the data appearing the top 30 PCs (chosen via Scree plots in Fig. S~\ref{fig:scree1}), a UMAP shows considerable overlap between the clusters of real and synthetic abstracts. This suggests that dimensionality reduction methods that utilize the full set of PCs may fail at distinguishing real and AI-generated samples when this variability is captured in a single PC.

Similar shifts are seen across other synthetic text and image datasets when compared to a real baseline. The results in Table~\ref{table:LDA_Embeddings} indicate that there is typically a linear classifier that can separate real and AI-generated data with remarkable accuracy $(>98\%)$, including the GenImage benchmark dataset \cite{genimage}. Of interest is one of the lower performers, where DNN embeddings can separate real cat images from the generations of a Denoising Diffusion Probabilistic Model (\texttt{DDPM}~\cite{ddpm}) with $92.7\pm1.41\%$ accuracy. The real images and the training dataset for \texttt{DDPM} are both sampled from the LSUN dataset \cite{yu2015lsun}. Compare this to the starker shift observed between the real baseline and cat images generated with more recent models (e.g. Stable Diffusion XL v1.0 (\texttt{SDXL}) \cite{podell2024sdxl} and \texttt{Open Dalle} \cite{OpenDalle}) that were trained on swaths more than just cat images. Our result suggests that while \texttt{DDPM} fails to learn true distribution of its own training set, the `higher fidelity’ models generate data whose embeddings lie further from the signal subspace of the LSUN cat data. 

%We see similar shifts across other experiments. We task three image generation models --- a Denoising Diffusion Probabilistic Model (\texttt{DDPM})~\cite{ddpm}, Stable Diffusion XL v1.0 (\texttt{SDXL})~\cite{podell2024sdxl}, and \texttt{Open-Dalle}~\cite{OpenDalle} --- to produce images of cats. Using \texttt{DFN} as the FE, we see that the generated images are shifted from our reference sample of cat images from the LSUN dataset~\cite{yu2015lsun} (Fig.~\ref{fig:MAIN2}A). An LDA classifier achieves $98.8 \pm 0.38\%$ binary test accuracy when comparing the real and fake cat images. Of particular note is those images produced by the \texttt{DDPM} model which was trained exactly on the cat class of LSUN. Our findings show that \texttt{DDPM} fails to reproduce the distribution of its own training data, with LDA achieving $92.7 \pm 1.42\%$ test accuracy in classifying between the two sources. For the more recent models, \texttt{SDXL} and \texttt{Open-Dalle}, that are trained on swaths more data, the shift from the real baseline is more pronounced. On GenImage \cite{genimage} (Fig.~\ref{fig:MAIN2}A), a benchmark dataset for AI-image detection, the test accuracy for classifying ImageNet \cite{imagenet} data against images from eight recent generative models, was $98.3\% \pm 0.07$. For NLP, we task language models with answering questions posted on StackExchange Q\&A forums, obtaining a $99.0\%$ classification between real and fake responses.


\subsubsection*{Embeddings are sensitive to generative techniques}\label{sensitivity}
Differences in generative techniques, such as model choices and prompting method, changes the resulting generated data~\cite{sahoo2024systematic, rafailov2023direct}. These choices lead to shifts in the sampling distributions that are observable when viewed through a consistent FE. While unsupervised clustering techniques can often recognize such shifts, they become pronounced with supervision (see Fig.~\ref{fig:MAIN2}A). This section establishes a proof-of-concept towards the forensic analysis of synthetically generated data by comparing the DNN embeddings of different synthetic samples against each other — extending the comparisons against real data and showing that DNN embeddings can provide analytic tools for generative models.

%This section establishes a proof-of-concept towards the forensic analysis of synthetically generated data by comparing the DNN embeddings of different synthetic samples against each other --- extending the comparisons against real data. In turn, DNN embeddings can provide analytic tools for generative models.

%Given a sample from one of several understood distributions, we can trace through the embedded representations to determine if it is real or synthetic, and in the latter case, distinguish generative parameters. 

\noindent\textbf{Generative DNA (gDNA).} We find evidence that different generative models have identifying ‘gDNA’ for source determination. As a continued example, consider cat images from the LSUN dataset compared to ones that are produced by DDPM, SDXL, and Open Dalle. We find that unsupervised clustering creates two groups that can be separated along PC1: the outputs of SDXL with Open Dalle and the outputs of DDPM with the LSUN cat data. This suggests that when measured against the task of generating cat images, the vectors produced by the FE relate the outputs of Open Dalle more closely to that of SDXL than DDPM. In fact, this captures the fact that Open Dalle is a fine-tuning of SDXL! This sensitivity is captured in other model families as well; different versions of Stable Diffusion generate similar images and translations produced by language models in the same family will generate similar text. See Supplementary Text for details.

In the case of natural language, we find that LLMs have their own writing styles which surface when they are prompted without certain constraining criteria. To test this, we asked three LLMs --- \texttt{Llama-2 70B}~\cite{touvron2023llama2openfoundation}, \texttt{Mixtral 8x7B}~\cite{jiang2024mixtralexperts}, and \texttt{Falcon 40B}~\cite{almazrouei2023falconseriesopenlanguage} --- to generate responses to questions posted on StackExchange~\cite{h4stackexchange}. Comparing these answers to user-posted replies, we learned that the vectors produced by the FE could be used to reliably predict which of the four sources a given answer came from ($90.7\pm0.27$ average accuracy). Hence, upon vectorization, each sample is concentrated in a different region of the ambient embedding space. This indicates that different LLMs are learning different distributions to model language, each shifted from the next. To understand the effects of constraint criteria, we compared translations produced by different models in both the long- and short-form regimes (c.f. Fig.~\ref{fig:short-long}). In the long-form case, we were able to disentangle the English translations of German sports articles with $93.2\%$ test accuracy. Contrastingly, we had significant challenge classifying the translations of small phrases appearing in the United Nations Parallel Corpus~\cite{ziemski-etal-2016-united}. Nor did we find significant separation between the machine translations and the provided human translations in the dataset, suggesting that the samples of machine translations overlap with the human translations when mapped into the ambient embedding space. We suspect that the perceived overlap is a consequence of the restrictive nature of short-form translations. With little opportunity to reveal their internal biases, the different linguistic styles associated and human or machine translation are not reflected when vectorized by the FE. We are unaware of analogous constraints in the image domain, finding that the images produced by each generative model cluster in separable regions of the ambient embedding space. 

%We find that different generative models have identifying `mDNA' for source determination. Returning to our results on StackExchange, supervised LDA can be used to predict whether an answer is user-written, or created by \texttt{Llama-2 70B}, \texttt{Mixtral 8x7B}, or \texttt{Falcon 40B} with an average overall accuracy of $90.7\%$. The presence of mDNA is further supported when we asked language models --- \texttt{Mixtral-8x7B}, \texttt{nllb-3.3B}, and \texttt{mt-opus-de-en}~\cite{tiedemann-thottingal-2020-opus} --- to translate 5,000 sports articles from German to English. We compare the  of the resulting outputs, correctly identifying the machine translator of a given article with $93.2\%$ test accuracy using a supervised classifier trained on the vectorizations from \texttt{Mistral 7B}. We suspect that our ability to detect mDNA in different textual settings is due to the long-form nature of the generative tasks which give the language models room to reveal their internal biases. In the short-form regime, the models have less flexibility due to the constraints of the response length. Asking language models to translate small phrases appearing in the United Nations Parallel Corpus~\cite{ziemski-etal-2016-united}, our techniques do not identify significant separation between machine and human responses in this translation task. See Fig.~\ref{fig:short-long} for a comparison of sample lengths between MLSUM and the UNPC. On the GenImage benchmark, LDA achieves $96.1 \pm 0.18$ test accuracy in classifying images from all nine sources, eight models plus ImageNet, further supporting the presence of mDNA.

Prompting techniques also influence the gDNA of AI data. Asking \texttt{Llama-2 70B} to generate economics abstracts with two different instructions, we learned that the vectorized samples were shifted between the two prompts. The intuitive changes that we see when prompting language models to be more thorough in explanations, listing accomplishments, or connecting to other research trends are preserved by the machinery of the FE. By mapping these changes in the embedded space, we can precisely study the effects of swapping our prompts.

%\noindent\textbf{Prompting and Lineage.} The vectors produced by FEs can also detect shifts in generative content caused by changes in prompting techniques. Using two different prompts to generate economics abstracts created with \texttt{Llama-2 70B}, Fig.~\ref{fig:MAIN2}A shows that text vectorizations preserve enough signal to almost entirely separate the sample distributions corresponding to each prompt, with LDA achieving a test accuracy of $92.0 \pm 1.46\%$ at classifying the generative outputs from the two prompts. Section \ref{section:explaining} shows that we can analyze this vectorized data to quantitatively verify and further refine observations we make by manual inspection.

%Distributions of outputs for related models are more closely aligned to the distributions of outputs for unrelated ones. The clusters observed for cat images through PCA in Fig. \ref{fig:MAIN2}A show that the outputs generated by \texttt{Open Dalle} and \texttt{SDXL} cluster along PC1, the former model being a fine-tuning of the latter. A second cluster is formed along PC1 between \texttt{DDPM} and the reference LSUN cat images, which is explained by the fact that \texttt{DDPM} was trained using LSUN. In the supervised setting, we observe lower accuracy when classifying images within these two clusters than across them, with $90.1 \pm 1.63\%$ in the first case (\texttt{SDXL} versus \texttt{Open-Dalle}), $92.7 \pm 1.41\%$ in the second (\texttt{DDPM} versus LSUN), $100 \pm 0.0\%$ test accuracy across clusters. Sensitivity to model lineage is evident in the GenImage benchmark as well, where the lowest LDA binary classication accuracy ($94.85\% \pm 0.40$) is between the two Stable Diffusion models, versions 1.4 and 1.5.

\subsubsection*{Explaining distribution shifts via cluster regression}\label{section:explaining}

Having observed different modalities between the various sources of AI-generated data and their real counterparts, we can begin explaining some of the more nuanced shifts with linear regressions. To do this, we pass our data through simple and interpretable indicator functions to isolate specific features and then regress these outputs against the numerical features obtained by PCA or LDA. Regarding the AI-generated abstracts, we found that the language model tended towards using words like `innovation,’ `valuable,’ and `insight’ when compared to those written by real scientists ($R^2=0.47$). This was also noticed in generating the economics abstracts --- prompting the language model to highlight the achievements led to an increased use of this boosted language ($R^2=0.41$). In the case of StackExchange, we find that the frequency of special characters contributed to the variance observed along PC1 $(R^2=0.56)$. While we hypothesize this feature is associated with technical topics like math or programming, PCA provided an organization of our data with prose on one end and technical formatting on the other. Further regressions are provided in the Supplementary Text. 




%Performing linear regressions on observed PCA and LDA clusters enables a more nuanced explanations for these modes.
%We build simple indicator functions for latent textual data that correspond to easily interpretable attributes. Using these indicator functions as explanatory variables, we predict the numerical features given by PCA or LDA. 
%A list of regressions can be found in the Supplementary Materials. Among our findings, we learn that the separation between real abstracts and fake ones (PC4) produced by \texttt{Llama-2 70B} is partially explained by the presence of filler words that stress the importance of the proposed work, with $R^2=0.47$ when analyzing abstracts across five different subject areas.  
%In our five topic arXiv dataset, this separation occurs along PC4 and we get an $R^2$ of $0.47$ between the explanatory and response. 
%Focusing solely on economics abstracts, a similar choice of words gives partial explanation for the separation of real and fake (PC1) with $R^2=0.51$. %, indicating that some of the shift between the real and AI-generated samples can be explained by the LLM's tendency to generate abstracts containing self-praising prose.
%Alternately, regressing PC1 of the economics abstracts on whether the length was over $1500$ characters, we get an $R^2$ of $0.57$, indicating that considerable variation between our real and synthetic abstracts %, from either prompt, 
%is explained by length of the text, with synthetic abstracts being typically longer than real ones. In the Stack Exchange data, the separation between the real and fake data occurred along the first linear discriminant (LD). We hypothesize that for question-answering, language models explicitly insert `helpful' words and phrases. In this case, our indicator variable gives a weaker explanation to the difference between real and AI responses with $R^2=0.29$.

%We can also explore other features extracted from the embedded data. In this case for example, we find that PC1 is partially explained by the presence of special characters ($R^2=0.56$). We hypothesize that this is associated with notions of computer science and mathematics.

\subsubsection*{Filtering AI-generations via anomaly detection}
In our previous examples, we had equal parts real and AI-generated data and the shifts we cared about were observed in the top principal components. We test our ability to use isolation forests for detecting AI-responses to StackExchange data when we only have a few samples generated by \texttt{Llama-2 70B}. The scatterplots in Fig.~\ref{fig:MAIN3} show that while the synthetic responses fit among the real data in the top few PCs, they are revealed as outliers when we consider more principal components. Empirically, we find that our sensitivity of detecting fake responses with this method is related to the proportion of fake answers; too many contaminates and you create a new cluster, too few and their signal will be buried.

%relationship between the relative amounts of real ($N$) and fake ($M$) responses and our sensitivity of detecting fake responses as outliers in our data. With very little contamination, the most sensitive predictors are those which use smaller amounts of reference data ($N<500$). As we increase the size the amount of contamination, the most sensitive predictors become those with larger reference samples of real data.

\begin{figure} % Do NOT use \begin{figure*}
	\centering
	\includegraphics[width=0.6\textwidth]{figures/sci-figs/FIG1_DRAFT.jpg} % for an image file named example_figure.*
	% Pick an appropriate width - in print, figures are usually one or two columns wide, which can
	% be approximated by 0.3\textwidth or 0.6\textwidth respectively. Use appropriate label sizes.

	% Captions go below figures
	\caption{\textbf{Dimensionality reduction on embedded features reveals high-level structure.}
		(\textbf{A}) Framework of our techniques. The full neural network begins by engineering a vector representation of the data through its feature embedder (FE). The embedded data is then passed through an interchangeable machine learning layer. Principal component analysis (PCA) is highlighted as an example technique to understand the representation produced by the FE. (\textbf{B}) PCA is used on embedded data to capture high-level semantics of observed data. Left: Top three principal components (PCs) on Spanish and Russian news articles, including Russian-to-Spanish machine translations. These features automatically separate Spanish and Russian texts, sports and economics data, and the native Spanish articles from the translated ones. Right: Top three PCs of scientific abstracts from arXiv.org and synthetic ones from Llama-2 70B. These features can be used to identify physics, computer science, or quantitative biology papers, regardless of origin.  (\textbf{C}) Kernel density estimates on selected PCs of the same data in (B). Embedded data forms interpretable clusters along different PCA dimensions.}
	\label{fig:MAIN1} % give each figure a logical label name
\end{figure}

\begin{figure} % Do NOT use \begin{figure*}
	\centering
	\includegraphics[width=0.6\textwidth]{figures/sci-figs/FIG2_DRAFT.jpg} % for an image file named example_figure.*
	% Pick an appropriate width - in print, figures are usually one or two columns wide, which can
	% be approximated by 0.3\textwidth or 0.6\textwidth respectively. Use appropriate label sizes.

	% Captions go below figures
	\caption{\textbf{Embedded data to distinguish real and fake data.}
		(\textbf{A}) DNN embeddings of AI-generated data alongside real data, after dimensionality reductions. In all cases, PCA identifies a shift between real and synthetic content. Supervised learning with linear discriminant analysis (LDA) can separate all classes of data. I. User-posted StackExchange answers and those written by three different language models (Mistral 8x7B, Llama-2 70B, and Falcon 40B). Embeddings by Mistral 7B. II. Real cat images from the LSUN dataset and images produced by three image generation models (DDPM, Stable Diffusion, and Open Dalle). Embeddings by Apple’s Data Filtering Network. III. Real economics abstracts and two sets of synthetic ones created by Llama-2 70B using different prompting methods. Embeddings by Mistral 7B. IV. Real and AI-generated images from the GenImage dataset containing data produced by nine separate generative models. Embeddings by Apple’s Data Filtering network.  (\textbf{B}) Dimensionality reduction techniques on embedded arXiv abstracts in across five subjects, along with synthetic abstracts produced by Llama-2 70B. Embeddings by Mistral 7B. Left: Dimensionality reduction using UMAP on the top 30 PCs of the embedded data. Middle: PCs 2 and 4. Right: LD2 and 5.}
	\label{fig:MAIN2} % give each figure a logical label name
\end{figure}

\begin{figure} % Do NOT use \begin{figure*}
	\centering
	\includegraphics[width=0.6\textwidth]{figures/sci-figs/FIG3_DRAFT.jpg} % for an image file named example_figure.*
	% Pick an appropriate width - in print, figures are usually one or two columns wide, which can
	% be approximated by 0.3\textwidth or 0.6\textwidth respectively. Use appropriate label sizes.

	% Captions go below figures
	\caption{\textbf{Outlier detection to filter AI content.}
        We contaminate samples of user-written StackExchange responses with a small number of answers generated by Llama-2 70B, embedded using the Mistral 7B language model. 
		(\textbf{A}) Example with 1000 user replies and 10 AI-written answers. The synthetic responses embed among the real ones when looking at the top PCs, but they are outliers when examining higher PCs. (\textbf{B})We use isolation forests on the PCs to predict whether AI responses correspond to outliers in the embedded data. Using at most 50 PCs across 50 seeds, we report median AUROC scores as we vary the size of the reference sample (N) and the number of AI contaminants. }
	\label{fig:MAIN3} % give each figure a logical label name
\end{figure}
